Scalable Local Timestepping on Octree Grids

Numerical solutions of hyperbolic partial differential equations(PDEs) are ubiquitous in science and engineering. Method of lines is a popular approach to discretize PDEs defined in spacetime, where space and time are discretized independently. When using explicit timesteppers on adaptive grids, the use of a global timestep-size dictated by the finest grid-spacing leads to inefficiencies in the coarser regions. Even though adaptive space discretizations are widely used in computational sciences, temporal adaptivity is less common due to its sophisticated nature. In this paper, we present highly scalable algorithms to enable local timestepping (LTS) for explicit timestepping schemes on fully adaptive octrees. We demonstrate the accuracy of our methods as well as the scalability of our framework across 16K cores in TACC's Frontera. We also present a speed up estimation model for LTS, which predicts the speedup compared to global timestepping (GTS) with an average of 0.1 relative error.

==> ad.tex <==
\subsection{Experiments}
Experiments performed in \Frontera~ are executed in the following module environment. 
\begin{verbatim}
Currently Loaded Modulefiles:
  1) intel/19.0.5        4) python3/3.7.0
  2) impi/19.0.5         5) autotools/1.2
  3) petsc/3.12          6) cmake/3.16.1
\end{verbatim}

\subsubsection{Scaling}
The configuration file for scaling tests is provided  under the repository folder \texttt{NLSigma/par/nlsmA.par.json}. The detailed description for each parameter in the file is provided as a comment in the parameter file. 

In order to run the cases, please use:
\begin{verbatim}
ibrun -np <mpi tasks> 
  ./NLSigma/nlsmSolverNUTS 
      <par file> <ts_mode>
\end{verbatim}

\subsubsection{NLSigma}
All the experiments presented in the paper, use the source code in the \texttt{NLSigma} folder. To build the code, 

\begin{verbatim}
mkdir build
cd build
ccmake ../.
make nlsmSolverNUTS -j4
\end{verbatim}

To enable the profile counters, \texttt{ENABLE\_DENDRO\_PROFILE\_COUNTERS} on, and to switch between linear and non-linear wave propagation \texttt{NLSM\_NONLINEAR} off and on correspondingly.

nlsmSolverNUTS take two arguments, the first argument is the path to the parameter file, the second argument is the timestepping mode, which is an integer value, 
\begin{itemize}
    \item 0 : perform \nuts~ timestepping. 
    \item 1 : perform \uts~ timestepping. 
    \item 2 : perform single \nuts~ step and required steps by the uniform timestepping, each the same time. 
    \item 3 : perform 2 until we reach the simulation end time specified on the parameter file. 
\end{itemize}{}

\subsection{\Frontera~ compute node configuration}
\begin{verbatim}
    Architecture:          x86_64
    CPU op-mode(s):        32-bit, 64-bit
    Byte Order:            Little Endian
    CPU(s):                56
    On-line CPU(s) list:   0-55
    Thread(s) per core:    1
    Core(s) per socket:    28
    Socket(s):             2
    NUMA node(s):          2
    Vendor ID:             GenuineIntel
    CPU family:            6
    Model:                 85
    Model name:            Intel(R) Xeon(R)
    Platinum 8280 CPU @ 2.70GHz
    Stepping:              7
    CPU MHz:               2700.000
    BogoMIPS:              5400.00
    Virtualization:        VT-x
    L1d cache:             32K
    L1i cache:             32K
    L2 cache:              1024K
    L3 cache:              39424K
    
    MemTotal:       195920208 kB
    MemFree:        168962328 kB
    MemAvailable:   168337408 kB
\end{verbatim}


==> inuts.tex <==
%\subsection{Implicit non uniform timestepping}
